Layer-wise Fast Adaptation for End-to-End Multi-Accent Speech Recognition

Accent variability has posed a huge challenge to automatic speech recognition~(ASR) modeling. Although one-hot accent vector based adaptation systems are commonly used, they require prior knowledge about the target accent and cannot handle unseen accents. Furthermore, simply concatenating accent embeddings does not make good use of accent knowledge, which has limited improvements. In this work, we aim to tackle these problems with a novel layer-wise adaptation structure injected into the E2E ASR model encoder. The adapter layer encodes an arbitrary accent in the accent space and assists the ASR model in recognizing accented speech. Given an utterance, the adaptation structure extracts the corresponding accent information and transforms the input acoustic feature into an accent-related feature through the linear combination of all accent bases. We further explore the injection position of the adaptation layer, the number of accent bases, and different types of accent bases to achieve better accent adaptation. Experimental results show that the proposed adaptation structure brings 12\% and 10\% relative word error rate~(WER) reduction on the AESRC2020 accent dataset and the Librispeech dataset, respectively, compared to the baseline.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> backup/content/expr.tex <==
\subsection{Setup}
\label{sec:expr_setup}

\subsubsection{Dataset}
\label{sec:expr_dataset}

Our experiments are conducted on the Accented English Speech Recognition Challenge 2020~(AESRC2020) dataset~\cite{AESRC2020Datasetshi} and the Librispeech corpus~\cite{panayotovLibrispeechASRCorpus2015}. 
AESRC2020 contains a training set for 8 English accents in England~(UK), America~(US), China~(CHN), Japan~(JPN), Russia~(RU), India~(IND), Portugal~(PT) and Korea~(KR), with 20-hour data for each accent, however two more accents Canada~(CAN) and Spain~(ES) are included in test set while cv set has eight accents. 
Librispeech contains a 960-hour training set, while dev-clean/other~(dev~c/o) and test-clean/other~(test~c/o) are used for standard tests.
% Both Librispeech and AESRC2020 datasets are used for evaluation in our experiments.
% Librispeech test sets are used as standard test data, consisting of dev-clean/other~(dev~c/o) and test-clean/other~(test~c/o) subsets.
% AESRC2020 test sets are used as accented test data, consisting of a cross validation~(cv) set and a test set.
% Note that the cv set in the AESRC2020 dataset has the same number of accents as the training set, while the test set has two more accents that are unseen in the training set, i.e.~Canada~(CAN) and Spain~(ES).
We report the word error rate~(WER) on all evaluation sets.

\subsubsection{E2E based Baseline}
\label{sec:expr_baseline}

% Our ASR models are trained with 160 hours AESRC2020 data and 960 hours Librispeech data, where we treat Librispeech data as general data and the AESRC2020 data as accented data. 
For acoustic feature extraction, 80-dimensional fbank features are extracted with a step size of 10ms and a window size of 25ms, and utterance-level cepstral mean and variance normalization (CMVN) is applied on the fbank features.
For language modeling, the 500 English Byte Pair encoding~(BPE)~\cite{subword_bpe_Kudo_2018} subword units are adopted.
For E2E ASR, we adopt the transformer with the configuration of a 12-layer encoder and a 6-layer decoder ~\cite{attention_is_all_you_need,speech_transformer}, where each self-attention layer has an attention dimension of 512 and 8 heads.
SpecAugment~\cite{park_specaug_2019} is also applied for data augmentation during training.
% The baseline was trained for 50 epochs by the ``noam" optimizer~\cite{attention_is_all_you_need} with 25,000 warmup steps.
During decoding, the CTC module is used for score interpolation~\cite{JointCTCAttentionBased_kim_2017} with a weight of 0.3, and a beam width of 10 is applied for beam searching.
All models are built using the ESPnet toolkit~\cite{watanabeESPnetEndtoEndSpeech2018}.
% The final model for each experiment is obtained by averaging the last five epochs.

\subsection{Accent Identification and Embedding Extraction}
A pretrained time-delay neural network (TDNN)~\cite{tdnn_2015} based accent identification~(AID) model is used for extracting 256-dimension accent embeddings.
It accepts phone posteriorgram~(PPG) features as input and is trained to predict accent categories.
The accent embeddings are obtained from the penultimate layer output of the AID model.
% Training data include AESRC, Librispeech, and augmented speech data via text-to-speech (TTS).
More details about the AID model can be found in our accent identification system description~\cite{huangAISPEECHSJTUACCENTIDENTIFICATION} for the AESRC 2020 challenge~\cite{AESRC2020Datasetshi}.


\subsection{Exploration of Multi-Basis Adapter Layer}
\label{sec:expr_explore}

We first investigate the performance of the proposed multi-basis adapter layer architecture in Section~\ref{sec:multi_basis} with different injection positions, numbers of bases and types of bases.
% Our proposed methods have used step-by-step training. 
% A transformer baseline is pretrained as mentioned in Section~\ref{sec:baseline} and Section~\ref{sec:expr_baseline}.
% Next, adapter layers were injected into different encoder blocks and trained with the Adam~\cite{kingma2014adam} optimizer with learning rate equal to 1e-3.

% Here we explored different aspects of adapter layers described in Section~\ref{sec:multi_basis}.

\subsubsection{Position of Adapter Layer}
\label{sec:expr_position}

The performance of the baseline model in Section~\ref{sec:baseline} and our proposed models with 4-basis adapter layers are compared in Table~\ref{tab:layer_position}.
Different positions of the adapter layers are evaluated, including $\{1\}, \{6\}, \{12\}, \{1\text{-}6\}$, and $\{1\text{-}12\}$, where $\{m\text{-}n\}$ means injecting adapter layers into the $m^{\text{th}}${\raise.17ex\hbox{$\scriptstyle\sim$}}$n^{\text{th}}$ encoder blocks.
% Different injection positions of the adapter layers are evaluated, including $\{1\}, \{6\}, \{12\}, \{1\text{-}6\}$, and $\{1\text{-}12\}$, where $\{m\text{-}n\}$ means injecting adapter layers into the $m^{\text{th}}${\raise.17ex\hbox{$\scriptstyle\sim$}}$n^{\text{th}}$ encoder blocks.

% It is observed that all adapter layer-based models outperform the baseline.
For models with different positions of a single adapter layer injected at only one encoder block (lines~2{\raise.17ex\hbox{$\scriptstyle\sim$}}4), the performance becomes slightly worse as the injection position moves towards the last encoder block.
However, as the number of adapter layers increases, the WER is only on par with single adapter layer-based models.
This indicates that a single adapter layer injected in the first encoder block is already capable of adapting to various accents, while still keeping the parameter efficiency.
Therefore, in the following experiments, only one multi-basis adapter layer is injected in the first encoder block.

\setcounter{table}{0}
\begin{table}[H]
\centering
\caption{
Performance (WER) (\%) comparison of the multi-basis adapter layer positions and numbers.
}
\label{tab:layer_position}
\begin{tabular}{cc | cc cc}
\hline
\multirow{2}[2]{*}{Position} & \multicolumn{2}{c}{Accent} & \multicolumn{2}{c}{Libri} \\
\cmidrule(l{10pt}r{10pt}){2-3} \cmidrule(l{10pt}r{10pt}){4-5} 
& cv & test & dev c/o & test c/o \\
\hline
- & 6.54 & 7.61 & 5.64/11.43 & 6.31/11.68 \\
\{1\} & \textbf{5.91} & \textbf{6.82} & \textbf{{5.17/10.37}} & \textbf{{5.48/10.65}} \\
\{6\} & 5.91 & 6.89 & 5.23/10.41 & 5.51/10.73 \\
\{12\} & 6.08 & 7.08 & 5.20/10.67 & 5.74/10.97 \\
\hline
\{1-6\} & 5.85 & 6.82 & \textbf{5.21/10.39} & 5.65/10.79 \\
\{1-12\} & \textbf{5.82} & \textbf{6.78} & 5.23/10.27 & \textbf{5.61/10.69} \\
\hline
\end{tabular}
\end{table}

\subsubsection{The Number of Bases}
\label{sec:expr_number}

We then explore the impact of different bases numbers (ranging from 2 to 8) on the ASR performance.
% Here, different numbers from 2 to 8 of basis in the adapter layer were explored.
As shown in Table~\ref{tab:basis_number}, the WER is gradually decreased as the number of bases increases from 2 to 8.
% performance improvements if the number is larger than 1, and the performance is improved gradually with the increased basis number.
However, the performance gain is very limited when more than 4 bases are used, but more basis will result in more parameters.
%It has the best performance if the layer has 8 bases, since each basis corresponded to one accent in train set. 
%However 2 unknown accent Canada~(CAN) and Spain~(ES) could not fit the basis well.
%If only 2 or less basis were used in the adapter layer, results become considerably worse compared to 4 or 6 basis, due to the modeling ability of modules.
Considering the tradeoff between performance and model size, we adopt the 4-basis adapter layer in our following experiments.
% Accordingly 4-basis adapter layer is considered as a good balance between model accuracy and parameter size in the rest experiments.

\begin{table}[H]
\centering
\caption{
Performance (WER) (\%) comparison on different numbers of bases in one adapter layer.
}
\label{tab:basis_number}
\begin{tabular}{c cc cc}
\hline
\multirow{2}[2]{*}{\# Bases} & \multicolumn{2}{c}{Accent} & \multicolumn{2}{c}{Libri} \\
 \cmidrule(l{10pt}r{10pt}){2-3} \cmidrule(l{10pt}r{10pt}){4-5} 
 & cv & test & dev c/o & test c/o \\
\hline
- & 6.54 & 7.61 & 5.64/11.43 & 6.31/11.68 \\
% - & 6.54 & 7.61 & 5.64/11.43 & 6.31/11.68 \\
2 & 6.23 & 7.34 & 5.36/11.06 & 6.01/11.32 \\
4 & 5.91 & 6.82 & 5.17/\textbf{10.37} & \textbf{5.48/10.65} \\
6 & \textbf{5.89} & \textbf{6.81} & \textbf{5.14}/10.41 & 5.50/10.66 \\
8 & 5.78 & 7.01 & 5.20/10.43 & 5.52/10.71 \\
\hline
\end{tabular}
\end{table}
\setcounter{table}{3}

\begin{table*}[ht]
\centering
\caption{
Performance (WER) (\%) comparison of baseline system and different adaptation methods.
$\adapt_g$ denotes the proposed single-basis accent embedding layer adaptation model in Section~\ref{sec:ebd}, 
and $\adapt_m$ denotes the proposed multi-basis adaptation model introduced in Section~\ref{sec:multi_basis}, with injection only in the first encoder block.
}
\label{tab:final}
\label{tab:full}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ l ccccc ccccc | cc cc}
\hline
\multirow{2}[2]{*}{Model} &  \multicolumn{10}{c}{Accent Test Set} & \multicolumn{2}{c}{Accent} & \multicolumn{2}{c}{Libri} \\
 \cmidrule(l{10pt}r{10pt}){12-13} \cmidrule(l{10pt}r{10pt}){14-15} 
 &  US & UK & IND & CHN & JPN & PT & RU & KR & CAN & ES
& cv & test & dev c/o & test c/o \\
\hline
Baseline 
& 5.75 & 3.17 & 9.32 & 13.49 & 6.66 & 6.38 & 11.04 & 6.80 & 5.21 & 9.88 
& 6.54 & 7.61 & 5.64/11.43 & 6.31/11.68 \\
Finetune 
& 4.92 & 2.82 & 8.34 & 12.00 & 5.92 & 5.66 & 9.78 & 5.82 & 4.25 & 9.18 & 5.85 & 6.83 & 7.84/13.03 & 8.67/13.94 \\
$\adapt_g$
& 5.33 & 3.11 & 8.80 & 12.29 & 6.15 & 6.09 & 9.99 & 6.30 & 4.70 & 9.06
& 5.89 & 6.89  & 5.27/10.39 & 5.76/10.79 \\
$\adapt_m$
& 5.29 & \textbf{2.54} & 8.91 & 11.87 & 6.04 & 5.79 & 9.71 & 6.00 & 4.51 & 8.91
& 5.91 & 6.82 & 5.17/10.37 & 5.48/10.65 \\
$\adapt_g$ + $\adapt_m$
 &\textbf{4.88} & 2.57 & \textbf{8.38} & \textbf{11.54} & \textbf{5.73} & \textbf{5.60} & \textbf{9.71} & \textbf{5.70} & \textbf{4.21} & \textbf{8.51}
& \textbf{5.77} & \textbf{6.68} &  \textbf{4.73/10.22} & \textbf{5.32/10.61} \\
% WARN: switch cv/test to the last few lines
\hline
\end{tabular}%
}%
\end{table*}

\subsubsection{Different Types of Bases}
\label{sec:expr_type}

Table~\ref{tab:module_type} shows the performance of different bases types, including different connection modes (scale, shift, or both scale and shift) in Section~\ref{sec:multi_basis} and different projection module types in the bases.
DNN-based basis uses `Linear` whose encoded dimension is set to 128, while CNN-based basis uses `Conv2d` with a $5\times5$ kernel via 16 channels.
% For DNN-based bases, dense layers are used for the down and up projections, and the encoded dimension after down projection is set to 128.
% For CNN-based bases, Conv2d is used for the down and up projections with a $5\times5$ kernel with 16 channels.
% It can be seen that the shifting-only mode performs better than the scaling-only mode.
The best performance is achieved when both scaling and shifting are used.
This indicates that the shifting and scaling modes can benefit each other complementarily.
We further test different network types (DNN or CNN) in the bases implementation.
% DNN-based, Conv2d-based projection module types mentioned in Section~\ref{sec:multi_basis}, were used here to evaluate the results.
% It is observed that both network types achieve similar performance.
It is observed that CNN-based modules has insufficient ability to extract accent-related information.
In our final system, the DNN-based bases are used for consistency.

\setcounter{table}{2}
\begin{table}[t]
\centering
\caption{
Performance (WER) (\%) comparison of different projection module types and connections in the basis. 
}
\label{tab:module_type}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc cc cc}
\hline
\multirow{2}[2]{*}{\tabincell{c}{Network\\Type}} & \multirow{2}[2]{*}{\tabincell{c}{Connection\\Mode}} & \multicolumn{2}{c}{Accent} & \multicolumn{2}{c}{Libri} \\
\cmidrule(l{10pt}r{10pt}){3-4} \cmidrule(l{10pt}r{10pt}){5-6} 
 & & cv & test & dev c/o & test c/o \\
\hline
- & - & 6.54 & 7.61 & 5.64/11.43 & 6.31/11.68 \\
DNN & shifting-only & 5.96 & 6.91 & 5.22/10.41 & 5.51/10.78 \\
DNN & scaling-only & 5.95 & 6.99 & 5.23/10.44 & \textbf{5.46}/10.70 \\
DNN & both & \textbf{5.91} & \textbf{6.82} & \textbf{5.17/10.37} & 5.48/\textbf{10.65} \\
CNN & shifting-only & 6.12 & 7.11 & 5.16/10.61 & 5.67/11.10 \\
\hline
\end{tabular}%
}%
\end{table}

% \subsubsection{Training strategies on the predictor}
% \label{sec:expr_mtl}

% 
% During training, we found that if without any constraints, the distribution of interpolation coefficients $\al$ would rapidly reduce to a one-hot or two-hot vector, which greatly limits the adaptation capability of the adapter layer.
% Here, we explore two different ways to circumvent this issue.
% One is to first pre-train the predictor $p(\cdot)$ separately, and then freeze the predictor module when training the adapter layers.
% % kmeans clustering or multi-task regularization methods is used to avoid this problem.
% % The target label for pre-training the predictor is a probability on the clustering of accent embeddings.
% % As mentioned before in Section~\ref{sec:multi_task}, we faced module collapse during the training.
% % This means if no restriction was used on the predictor, the whole model overfitted the training data.
% % The predictor focused on one of all modules, in other words, other modules were not utilized.
% % So a pre-trained frozen predictor could be used, which is not suitable.
% A second approach is to regularize the predictor through multi-task learning~(MTL).
% We evaluated these strategies on the 4-basis adapter layer structure.
% % in Table~\ref{tab:mtl}.
% For MTL, the \textit{uniform} target label $\hal = 1 / n$, and the \textit{hard} target label (cluster assignment) mentioned in Section~\ref{sec:multi_task} are used for training.
% % Also a pre-trained predictor in Section~\ref{sec:multi_task} was able to solve this problem as the Table~\ref{tab:mtl} shown.

\subsection{Results Comparison of Different Adaptation Methods}
\label{sec:expr_full}

% Similarly, it achieves a lower WER than fine-tuning on accented data.
In this section, we present the detailed performance comparison of all proposed models and the baselines in Table~\ref{tab:full}.
Fine-tuning the baseline model for accented data is an intuitive way to perform adaptation on accented data, which is shown in the second line of Table~\ref{tab:full}. 
However, this is not feasible for some unseen accents like Spain~(ES), which is unavoidable during inference. On the other aspect, it degrades the performance on standard data, i.e.~Librispeech evaluation sets.
The gated adapter layer in Section~\ref{sec:ebd} is denoted as $\adapt_g$ in the table, which shows significant improvement on both Librispeech and accent datasets.
Denote by $\adapt_m$ the proposed multi-basis adapter layer introduced in Section~\ref{sec:multi_basis}, adapter layer $\adapt_m$ is injected only in the first encoder block, which consists of 4 bases that are structured by DNN-based projection modules.
% Furthermore, we concatenate adapter layers in \textbf{M0} and \textbf{M1} alternately to construct the final adapter layer, which is denoted as \textbf{M0+M1}.
% Furthermore, we also inject \textbf{M1} layer, regard
% Furthermore, \textbf{M1} Layer is also injected in the encoder block, with the input as the output of \textbf{M0} layer, which is denoted as \textbf{M0+M1}.
Furthermore, we combine $\adapt_g$ and $\adapt_m$ by computing the output as $h^i + \adapt_m(h^i + \adapt_g(h^i, z), z)$.
We observe that the final proposed method $\adapt_g$ + $\adapt_m$ consistently outperforms the baseline model which shows that the proposed method can learn accent-related information effectively and improve the robustness of speech recognition against accent variation.

\subsection{Visualization of Multi-Basis Adapter Layer}
\label{sec:expr_visual}

\begin{figure}[h]
\centering
\begin{subfigure}{0.2\textwidth}
\includegraphics[width=1.0\linewidth]{LaTeX/figs/boxplot/0.pdf}
\caption{Basis One}
\end{subfigure}
\begin{subfigure}{0.2\textwidth}
\includegraphics[width=1.0\linewidth]{LaTeX/figs/boxplot/1.pdf}
\caption{Basis Two}
\end{subfigure}
\begin{subfigure}{0.2\textwidth}
\includegraphics[width=1.0\linewidth]{LaTeX/figs/boxplot/2.pdf}
\caption{Basis Three}
\end{subfigure}
\begin{subfigure}{0.2\textwidth}
\includegraphics[width=1.0\linewidth]{LaTeX/figs/boxplot/3.pdf}
\caption{Basis Four}
\end{subfigure}
\caption{
Boxplot and violinplot visualization of interpolation coefficent distributions for each basis.
The vertical axis shows the interpolation coefficent $\alpha_i$, where $i$ is the basis index.
The horizontal axis is the accent categories.
% We plot all data in accent test by boxplot and violinplot to visualize the mean value of each accent on each module from subfigure $1$ to subfigure $4$.
% Adapter layer has four modules, and it is injected before the first transformer layer.
}
\label{fig:interpolation}
\end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.35\textwidth]{LaTeX/figs/tsne.png}
% \caption{t-SNE visualization of accent embeddings on the accent cv set.}
% \label{fig:tsne}
% \end{figure}

% Figure~\ref{fig:interpolation} shows the coefficient distributions on each basis from the 4-basis adapter layer model.
% Accents with large coefficients in each basis are assumed to be more correlated to that basis.
% It can be clearly seen that different bases capture a different set of highly correlated accents.
% For example, \textit{Basis Two} focuses mainly on extracting information about the Japanese~(JPN) accent, then the American~(US) and Chinese~(CHN) accents.
% The inherent correlation between different accents can be also revealed from this figure.
% For example, American~(US) and British~(UK) accents have consistently high correlations with \textit{Basis One}, and much lower correlations with other bases.
% Meanwhile, Portuguese~(PT) and Japanese~(JPN) accents have distinct preferences for bases: PT accent prefers \textit{Basis Four} while JPN accent prefers \textit{Basis Two}.
% % To better illustrate the correlation between different accents, we further visualize the accent embeddings extracted from the AID model via t-SNE~\cite{}, which is depicted in Figure~\ref{fig:tsne}.
% % Similar and consistent conclusions can be drawn from the visualization of accent embeddings.
% Results demonstrate that our proposed multi-basis adapter layer approaches can well-capture the accent-dependent information with the guidance of accent embeddings, thus improving the multi-accent ASR performance.


Figure~\ref{fig:interpolation} shows the coefficient distributions on each basis from the 4-basis adapter layer model.
Accents with large coefficients in each basis are assumed to be more correlated to that basis.
It can be clearly seen that different bases capture a different set of highly correlated accents.
For example, \textit{Basis Two} focuses mostly on extracting information about the Portuguese~(PT) accent, and then the American~(US) and Russian~(RU) accents.
The inherent correlation between different accents can be also revealed from this figure.
For example, American~(US) and British~(UK) accents have consistently high correlations with \textit{Basis One}, and much lower correlations with other bases.
Meanwhile, Indian~(IND) and Japanese~(JPN) accents have distinct preferences for bases: IND accent prefers \textit{Basis Four} while JPN accent prefers \textit{Basis Three}.
% To better illustrate the correlation between different accents, we further visualize the accent embeddings extracted from the AID model via t-SNE~\cite{}, which is depicted in Figure~\ref{fig:tsne}.
% Similar and consistent conclusions can be drawn from the visualization of accent embeddings.
Results demonstrate that our proposed multi-basis adapter layer approaches can well-capture the accent-dependent information with the guidance of accent embeddings, thus improving the multi-accent ASR performance.

==> backup/content/method.tex <==
\def \x {\mathbf{x}}
\def \y {{\mathbf{y}}}
\def \h {\mathbf{h}}
\def \a {\mathbf{a}}
\def \W {\mathbf{W}}

\newcommand{\adapt}{\mathcal{A}}
\newcommand{\hin}{\boldsymbol{h^i}}
\newcommand{\hac}{\boldsymbol{h^o}}
\newcommand{\zz}{\boldsymbol{z}}
\newcommand{\al}{\boldsymbol{\alpha}}
\newcommand{\hal}{\boldsymbol{\alpha^{\text{(ref)}}}}
\newcommand{\alk}{\alpha_k}
\newcommand{\ai}[1]{\alpha_#1}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{LaTeX/figs/final.pdf}
\caption{Schematic diagram of the proposed adapter layer. The adapter layer in (a) is optionally inserted in each encoder block, which is discussed in Section~\ref{sec:expr_position}. Here, $+$, $\times$, and $\odot$ denote summation, matrix multiplication, and element-wise product, respectively.}
\label{fig:pipeline}
\end{figure*}

\subsection{Pretrained transformer-based E2E ASR}
\label{sec:baseline}

The transformer is a sequence-to-sequence~(S2S) structure consisting of a multi-layer encoder and a multi-layer decoder~\cite{attention_is_all_you_need}.
The encoder takes acoustic features as input to be mapped into high-level representations $\h$.
The decoder network utilizes the encoded representation $\h$ with an attention mechanism and outputs the predicted tokens auto-regressively.
At each decoding step, the decoder emits the posterior probabilities of the next token given previous outputs.
We train the transformer model with the joint CTC-attention framework~\cite{JointCTCAttentionBased_kim_2017} to exploit the advantages from both CTC and attention-based models. 
The loss function is defined as below:
\begin{equation}
\label{eq:joint_ctc}
\begin{aligned}
\mathcal{L}_{jca} = \lambda_{ctc} \mathcal{L}_{ctc} + (1 - \lambda_{ctc}) \mathcal{L}_{s2s}
\end{aligned}
\end{equation}
where $\mathcal{L}_{ctc}$ and $\mathcal{L}_{s2s}$ are the CTC and S2S objective losses, respectively.
A tunable parameter $\lambda_{ctc} \in [0,1]$ is used to control the contribution of each loss.


% \subsection{Accent Classification}
% \label{sec:accent_classification}

% % \begin{figure}[h]
% % \centering
% % \label{fig:aidmodel}
% % \caption{Accent Idenfiticatoin}
% % \includegraphics[width=0.45\textwidth]{LaTeX/figs/aid.png}
% % \end{figure}

\subsection{Adapter Layer}
\label{sec:layer}

The E2E ASR model trained on common standard corpora usually lacks generalization on accented data due to the accent mismatch. % of training and evaluation data. 
Adapter layers are injected into the ASR encoder blocks to transform the accent-unrelated features into the accent-related space.
The architecture of the new ASR encoder with the proposed adapter layer is illustrated in Figure~\ref{fig:pipeline}(a).
The adapter layer, hereinafter denoted as $\adapt$, is used as a pre-processing to transform accent-unrelated features into accent-related features.
Denote by $\hin$ the input feature before the encoder block, $\zz$ the accent embedding, and $\adapt(\hin, \zz)$ the output feature in the accent-related space.
% The $\hac$ is wrapped to represent a no-op if necessary we wrap it with a residual connection as shown in Figure~\ref{fig:pipeline}(a).
The output feature $\adapt(\hin, \zz)$ is then wrapped into the encoder block by a residual connection ($+$) as shown in Figure~\ref{fig:pipeline}(a), to enable the original acoustic information to flow through later encoder layers.
Different types of adapter layers $\adapt$ are explored in the following sections: $\adapt_g$ in Section~\ref{sec:ebd} and $\adapt_m$ in Section~\ref{sec:multi_basis}.
% Different injection positions of the adapter layer are also explored in Section~\ref{sec:expr_position}, where each adapter layer has separate parameters.

\subsubsection{Gated Adapter Layer}
\label{sec:ebd}

The first scheme to attain the transform function follows our previous investigation in~\cite{tanAISPEECHSJTUASRSYSTEM}. 
As shown in Figure~\ref{fig:pipeline}~(b), a scaling factor $f(\zz)$ and a shifting factor $g(\zz)$ can be applied to the input feature for accent adaptation:
{\setlength\abovedisplayskip{4pt}
\setlength\belowdisplayskip{4pt}
\begin{equation}
\label{eq:ebd}
\adapt_g(\hin, \zz) = f(\zz) \odot \hin + g(\zz)
\end{equation}
}where $\adapt_g$ is the gated adapter layer, and $\odot$ denotes the element-wise product. $f(\zz)$ and $g(\zz)$ are separately generated by a single dense layer with $\mathrm{tanh}(\cdot)$ activation.

\subsubsection{Multi-basis Adapter Layer}
\label{sec:multi_basis}

The second scheme is to build a multi-basis adapter layer as in Figure~\ref{fig:pipeline}~(c).
% The adapter basis based technique has shown parameter efficiency and flexibility for domain adaptation in computer vision~\cite{adapter_cv_2017}, natural language processing~\cite{adapter_nlp_2019} and neural machine translation~\cite{adapter_nmt_2019}.
% At the same time, multi basis technique shows its potential on speaker\cite{wuWuchunyangIvector12016, tanCAT2015} or accent adaptation~\cite{Grace_Bastani_Weinstein_2018,jainMultiAccentAcousticModel2019}.
The multi-basis layer concatenates the output $B_k(\hin)$ from each basis with the corresponding interpolation coefficient $\alk$. 
Similar to Section~\ref{sec:ebd}, the scaling $F_k(\cdot)$ and shifting $G_k(\cdot)$ modules are used to transform the input $\hin$ into the accent-related space as shown in Figure~\ref{fig:pipeline}~(d), where $k = 1, 2, \ldots, n$ and $n$ is the number of adapter bases.
{\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\begin{equation}
\label{eq:adapter_layer}
\begin{aligned}
\adapt_m(\hin, \zz) = &\sum_{k=1}^n \ai{k} B_k(\hin) \\
                    = &\sum_{k=1}^n \ai{k} * \{ F_k(\hin) \odot \hin + G_k(\hin) \}
\end{aligned}
\end{equation}
}Note that one can also use scaling-only $\left(G_k(\hin)=\mathbf{0}\right)$ and shifting-only $\left(F_k(\hin)=\mathbf{0}\right)$ operations in the bases, which will be discussed in Section~\ref{sec:expr_type}.

\noindent\textbf{Projection Module}\quad To make the bases in Figure~\ref{fig:pipeline}~(d) simple and flexible, we propose a sandglass-style structure for $F(\cdot)$ and $G(\cdot)$ modeling: a down-projection network and a up-projection network with the non-linear activation $\mathrm{ReLU}(\cdot)$.
This architecture allows us to easily adjust the modules' capacity, depending on the complexity of the accents.
Additionally, we normalize the input of each adapter basis by LayerNorm~\cite{ba2016layernorm}.
% This normalization layer allows the module to learn the activation pattern of the adapter module to represent.

% Previous work on accessing $\alpha$ like~\cite{Grace_Bastani_Weinstein_2018} use one-hot vectors, however, is not suitable for unknown accents.
\noindent\textbf{Predictor}\quad Different from the one-hot accent vector that is commonly used in prior works on accent adaptation~\cite{Grace_Bastani_Weinstein_2018,yang2018joint}, here we adopt a soft assignment of bases by interpolating between all adapter bases dynamically.
To estimate interpolation coefficients $\al \in \mathbb{R}^n$ from accent embedding $\zz$, a predictor $p(\cdot)$ model is used, and give guidance on the usage of modules.
\begin{align}
\label{eq:predictor}
\al = \operatorname{SoftMax} (p(\zz)) \text{, where } 1 = \sum_{k=1}^n \alk
\end{align}
where the interpolation coefficients $\al = (\ai{1}, \ldots , \ai{n})$ are probabilities for multiple bases.
The predictor $p(\cdot)$ can be composed of several DNN layers.


% However, each affine module does not correspond to an individual accent, instead, linear composition of affine modules can represent the utterance's accent.

\subsubsection{Multi-task Regularization}
\label{sec:multi_task}

%% TODO: mention or not to mention here?
% For pretraining, we first cluster the accent embeddings using kmeans, and then take the cluster results as the target of $\alpha$ to pretrain the predictor.
% More skillfully, a multi-task training~\cite{luMoELuyizhou2020} is proposed to utilize both ASR and Predictor.
% The target $\hat{\alpha}$ to this $\mathcal{L}_{PG}$, can be defined as (1) use a uniform probability from all modules. (2) use the clustering results as the label.

During training, we found that, without any constraints, the distribution of interpolation coefficients $\al$ would rapidly reduce to a certain basis for all accents, which greatly limits the adapter layer's adaptation capability.
% Here, we explore two different ways to circumvent this issue.
Thus, we apply the multi-task learning~(MTL) scheme to utilize the loss from an auxiliary task, i.e.~the predictor in Section~\ref{sec:multi_basis}, to regularize the training of both ASR and predictor models.
% , which is usually used as a regularization strategy to improve the main task performance, to restrict the predictor.
An auxiliary loss from the predictor is introduced to the ASR loss $\mathcal{L}_{jca}$, and then the final loss $\mathcal{L}_{mtl}$ for the entire system is calculated as:
% Multi-task learning based regularization methods introduce another loss from the predictor model in addition to the ASR loss $\mathcal{L}_{jca}$.
% Denote by $\hat{\alpha}$ the target label of predictor outputs $p(\zz)$, then the final loss $\mathcal{L}_{mtl}$ for the entire system is written as:
{\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
\begin{equation}
\label{eq:mtl_loss}
\begin{aligned}
\mathcal{L}_{mtl} = \mathcal{L}_{jca} + \gamma_{mtl} \mathcal{L}_{\text{MSE}} (\hal, \al)
\end{aligned}
\end{equation}
}where $\hal$ is the target label of the predictor outputs $p(\zz)$, $\al$ is the output of the predictor, and $\gamma_{mtl}$ is a hyperparameter to control the contribution of the predictor loss.
%When $\gamma_{mtl} = 0$, the interpolation coefficients is not confined.
The target label $\hal$ is obtained via the clustering of accent embeddings extracted from the pretrained AID model.
The number of clusters is set to $n$, and here the K-means algorithm is adopted.
% The target probabilities $\hat{\alpha}$ are predefined in two ways.
% First is to set each probability equal, $\hat{\alpha} = \frac{1}{\text{\# Modules}}$. Second is to use the kmeans cluster target as the probability $\hat{\alpha} = {0,1,0,0}$.

% During training, we found that if without any constraints, the distribution of interpolation coefficients $\al$ would rapidly reduce to a one-hot or two-hot vector, which greatly limits the adaptation capability of the adapter layer.
% Here, we explore two different ways to circumvent this issue.
% One is to first pre-train the predictor $p(\cdot)$ separately, and then freeze the predictor module when training the adapter layers.
% kmeans clustering or multi-task regularization methods is used to avoid this problem.
% The target label for pre-training the predictor is a probability on the clustering of accent embeddings.
% As mentioned before in Section~\ref{sec:multi_task}, we faced module collapse during the training.
% This means if no restriction was used on the predictor, the whole model overfitted the training data.
% The predictor focused on one of all modules, in other words, other modules were not utilized.
% So a pre-trained frozen predictor could be used, which is not suitable.
% A second approach is to regularize the predictor through multi-task learning~(MTL).
% We evaluated these strategies on the 4-basis adapter layer structure.
% in Table~\ref{tab:mtl}.
% For MTL, the \textit{uniform} target label $\hal = 1 / n$, and the \textit{hard} target label (cluster assignment) mentioned in Section~\ref{sec:multi_task} are used for training.
% Also a pre-trained predictor in Section~\ref{sec:multi_task} was able to solve this problem as the Table~\ref{tab:mtl} shown.


==> backup/old---expr.tex <==

\subsection{Setup}

\subsubsection{Dataset}
\label{sec:dataset}

% Evaluation data includes accents that appears inside the train set and two more accents, Canadian and Spain which are outside the train set. For the sake of simplicity, we focus on accented English only. Nevertheless, we believe that our proposed approach will also be helpful in dealing with accented speech from other languages.

Our experiments are conducted on the Accented English Speech Recognition Challenge 2020~(AESRC2020) dataset~\cite{AESRC2020Datasetshi} and Librispeech corpus~\cite{panayotovLibrispeechASRCorpus2015}. 
The AESRC2020 training data was collected from speakers with eight accents in England~(UK), America~(US), China~(CHN), Japan~(JPN), Russia~(RU), India~(IND), Portugal~(PT) and Korea~(KR). There is a total of 160 hours multi-accent data in AESRC2020 training set, and 20 hours data for each accent. It is noted that in the official test set of AESRC2020, two additional accents are are reserved as unseen accented data only for evaluation, i.e. from Canada~(CAN) and Spain~(ES), and we report the WER results for these all ten accents in AESRC2020. Besides we also evaluate our system on the Librispeech dev \& test set to observe the system performance on the general data.

\subsubsection{Experimental baseline}
\label{sec:expr_baseline}
%%TODO: accent160 or accent20 is needed or not?
Our ASR models are trained with 160 hours AESRC2020 data and 960 hours Librispeech data, where we treat Librispeech data as general data and the AESRC2020 data as accented data. For acoustic features, 80 dimensional log-mel filterbanks are extracted with a step size of 10ms and window size of 25ms, and utterance-level CMVN is applied on the fbank features.
We use 500 English Byte Pair encoding~(BPE)~\cite{subword_bpe_Kudo_2018} subword units as our modeling units.

ESPNet toolkit~\cite{watanabeESPnetEndtoEndSpeech2018} is used to train our baseline model. A 12-layer encoder and a 6-layer decoder transformer~\cite{attention_is_all_you_need}, and each self-attention module has an attention dimension of 512 and 8 heads.
Also SpecAugment~\cite{park_specaug_2019} is applied for all data through out our experiments. 
The baseline was trained for 50 epochs, and the batch size is set to 24 with accumgrad 2. This is equivalent to set the batch size with 48.
``noam" optimizer~\cite{comparative_study_transformer_rnn_2019} with the 25,000 warmup steps, and an initial transformer learning rate of 10 was used.
During decoding, a multi-task CTC is used with the weight of 0.3, and the beam search with the size of 10 is applied.
The final model for each experiments was obtained by averaging the last five epochs.

%% Analysis


\subsection{Evaluation of accent adapter layer}
\label{sec:expr_eval}

%% Adaption work
According to previous work
~\cite{tanCAT2015,luMoELuyizhou2020,adapter_cv_2017}, the adapters should be added by a step-by learning.
In the first step, a baseline transformer is trained with both non-accent data and accent data. 
In the second step, adapter layer was injected within frozen transformer. 
% However, adapted features can not directly pass to old transformer layer, as they are trained to fit non-accent data more. 
And then we unfreeze all model parameters to fine-tune transformer parameters to fit both accent and non-accent data.

\begin{table*}
\centering
\caption{
Performance (WER) (\%) comparison of baseline system and different adaption methods.
}
\label{tab:final}
\begin{tabular}{ l ccccc ccccc | cc cc}
\hline
Model &  US & UK & IND & CHN & JPN & PT & RU & KR & CAN & ES
& cv & test & dev c/o & test c/o \\
\hline
Baseline &  5.75 & 3.17 & 9.32 & 13.49 & 6.66 & 6.38 &
11.04 & 6.8 & 5.21 & 9.88 & 6.54 & 7.61 & 5.6/11.4 & 6.3/11.6 \\
finetune &&&&&&&& \\
embedding &&&&&&&& \\
adapter &&&&&&&& \\
proposed &&&&&&&& \\
% WARN: switch cv/test to the last few lines
\hline
\end{tabular}
\end{table*}

Here, we compare our proposed model with different methods in Table \ref{tab:final}. 
The performance of baseline~(baseline) is at the first line. 
Results in accent cv set (6.54\%) and accent test set (7.61\%) shows the performance is not as good as we thought without accent information. 
We hypothesize that these will be optimized if accent information is appended.
From then on, we use this baseline as a pretrained model to get higher performance.
\textit{finetune} is to Fine-tuning baseline with each accent data of 20 hours.
\textit{embedding} relates to the method in Section \ref{sec:ebd} take an intuitive usage of accent embeddings, and shows consistency on both non-accent and accent evalution set.
% However, there is still potential of accent which is not fully exploited, as our Accent Identification(AID) system in Section \ref{sec:accent_classification} has an accuracy of 91\%, with 9\% errors.
\textit{adapter} relates to the method in Section \ref{sec:multi_basis}, 4 affine modules are used in each layer with 3 adapter layers injected. a MTL PG mentioned in \ref{sec:layer} was used to generate interpolation coefficents with $\gamma_{mtl} = 0.01$.

At the final line, we evaulate our best system with a concatenation of \textit{embedding} and \textit{adapter}. 
It is observed that the proposed adapter layers has better ability to modeling accent data without accuracy degradation on non-accent data. It can obtain a relevant 10\% WER reduction.

\subsection{Exploration the properties of adapter layer}
\label{sec:expr_explore}

In this section, we explored different properties of adapter layer described in Section \ref{sec:multi_basis}.

\subsubsection{Position of adapter layers}
\label{sec:expr_position}

In this section, we evaluate the impact on the position of adapter layers from $1, 3, 6, 9, 12$ and the influence if multiple adapter layers are injected in $\{1 \ldots 3\}$, $\{1 \ldots 6\}$, $\{1 \ldots 9\}$, $\{1 \ldots 12\}$.
From Table \ref{tab:layer_position}, the usage of multiple adapter layers yielded improvements over the best single layer before the second transformer encoder layer.
And the performance degraded when the adapter layer is inserted closer to the decoder.

\begin{table}[H]
\centering
\caption{
Performance (WER) (\%) comparison of the multi-module adapter layer positions and numbers. 
$\{m-n\}$ is to apply independent adapter layers into the encoder blocks from $m$ to $n$. 
Eight modules are used for each adapter layer. 
Layer type $A$ denotes the method mentioned in Section~\ref{sec:ebd}, $B$ denotes the method mentioned in Section~\ref{sec:multi_basis}.
}
\label{tab:layer_position}
\begin{tabular}{cc cc cc}
\hline
Layer & & \multicolumn{2}{c}{Accent} & \multicolumn{2}{c}{Libri} \\
Type & Position & cv & test & dev c/o & test c/o \\
\hline
- & - & 6.6 & 7.6 & 5.6/11.4 & 6.3/11.6 \\
A & \{1\} & 6.6 & 7.6 & 5.6/11.4 & 6.3/11.6 \\
B&\{1\} & 5.9 & 6.9 & -/- & 5.5/10.7 \\
B&\{6\} & 5.9 & 6.9 & -/- & -/- \\
B&\{12\} & 6.1 & 7.1 & 5.2/10.7 & 5.7/11.0 \\
B&\{1-6\} & 6.0 & 6.9 & 5.3/10.5 & 5.8/11.0 \\
B&\{1-12\} & 6.0 & 6.9 & -/- & -/- \\
\hline
\end{tabular}
\end{table}


% \subsubsection{Cluster Size}
\subsubsection{The Number of Modules}
\label{sec:expr_cluster_size}

Different quantities of affine modules from two to eight are explored in Table \ref{tab:cluster_size}. Single adapter layer is used.
It is obvserved that the results stay high performance as the number of modules reducing if the modules are considerably enough.
However, less modules means  less parameters that can simplify the whole model, so in later experiments we use \textbf{4} as the number of each adapter layer.

\begin{table}[H]
\centering
\caption{
Performance (WER) (\%) comparison of different numbers of modules.
Multi-module adapter layer is used and injected only in the first encoder block, before the convolution.
}
\label{tab:cluster_size}
\begin{tabular}{l cc cc}
\hline
\# Module & cv & test & dev c/o & test c/o \\
\hline
- & 6.6 & 7.6 & 5.6/11.4 & 6.3/11.6 \\
2 & 6.1 & 7.1 & - & - \\
4 & 5.9 & 6.9 & - & - \\
6 & 5.9 & 6.9 & - & - \\
8 & 5.9 & 7.0 & - & - \\
\hline
\end{tabular}
\end{table}



\subsubsection{Affine module type}
\label{sec:expr_module_type}

\begin{table}[H]
\centering
\caption{
Performance (WER) (\%) comparison of different affine module type. 
Eight affine modules are used in each adapter layer. 
Adapter layers are injected into \{1...6\} transformer layers.
}
\label{tab:module_type}
\begin{tabular}{l cc cc}
\hline
Type & cv & test & dev c/o & test c/o \\
\hline
- & 6.6 & 7.6 & 5.6/11.4 & 6.3/11.6 \\
DNN w LN shift & 5.9 & 6.9 & -/- & 5.5/10.7 \\
DNN w LN scale & 6.0 & 7.1 && \\
DNN w LN both & 5.8 & 6.8& -/- & -/- \\
DNN w/o LN shift &&&& \\
CNN w LN shift & 5.9 & 6.9 & -/- & -/-  \\
\hline
\end{tabular}
\end{table}

Here we explore how adapter basis type will influence the adaption with classic residual modules, including bottle-neck, MLP-based, Conv1d-based mentioned in \ref{sec:multi_basis}. The layers were trained with 8 affine modules, each of them represent one individual accent.
Results in Table \ref{tab:module_type} shows that adapter layer is not sensitive to different affine module types. 
The weight-only adaptation technique mentioned in \ref{sec:multi_basis} has similar performance compared with the weight-and-bias adaption, but way better than bias-only adaption.
In other words, affine module is captiable but 
So in the rest experiments, affine modules are set as a MLP-based affine module with weight-only technique.



\subsubsection{learnable interpolation coefficents}
\label{sec:expr_interpolation}

\begin{table}[H]
\begin{tabular}{c cc cc}
\hline
Position & cv & test & dev c/o & test c/o \\
\hline
- & 6.6 & 7.6 & 5.6/11.4 & 6.3/11.6 \\
no mtl &&&& \\
no mtl with init &&&& \\
+mtl uniform &&&& \\
+mtl hard &&&& \\
\hline
\end{tabular}
\end{table}

Tables shows that ...

\subsection{Visualization of Interpolation Coefficents}
\label{sec:expr_visual}

\begin{figure}[h]
\centering

\begin{subfigure}{0.22\textwidth}
\includegraphics[width=1.0\linewidth]{LaTeX/figs/0.png}
\caption{Module One}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}
\includegraphics[width=1.0\linewidth]{LaTeX/figs/1.png}
\caption{Module Two}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}
\includegraphics[width=1.0\linewidth]{LaTeX/figs/2.png}
\caption{Module Three}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}
\includegraphics[width=1.0\linewidth]{LaTeX/figs/3.png}
\caption{Module Four}
\end{subfigure}

\caption{Interpolation coefficents comparaison for each module. Adapter layer has 4 affine modules, and it is injected in the first transformer layer.}
\label{fig:interpolation}
\end{figure}

As shown in Figure \ref{fig:interpolation}, the interpolation coefficents varies from the accents. 
Different accent have different interpolation coefficents that is generate from Param Generator (PG) in Section \ref{sec:layer}.
Statistically, the UK accent features in the first column are caught by the \textit{affine module One}, and the KR accent features in the last column are caught by the \textit{affine module one} and \textit{two}.
However, even if two utterances are the same accent, their interpolation coefficents may differ according to the accent embedding, due to the pronunciation difference between speakers.

\begin{figure}[H]
\centering
\includegraphics[width=0.45\textwidth]{LaTeX/figs/tsne.png}
\caption{t-SNE for accent data and non-accent (librispeech) data}
\label{fig:tsne}
\end{figure}

In order to better understand how interpolation coefficents means to accents, accent embeddings are visulization in Figure \ref{fig:tsne}. 
The illustration shows that the interpolation coefficents somehow represent the correlation within a cluster.
%% BUG: does not means one-to-one map in cluster??

